Associated groups of symmetric quandles

In this paper, we investigate the structure of associated groups of symmetric quandles. Among other results, we explore the relationship between the associated group of a symmetric quandle and that of its underlying quandle. We provide a group-theoretic characterization of associated groups of symmetric quandles. Furthermore, we show that a symmetric quandle is embeddable if and only if its underlying quandle is embeddable, and we determine the abelianization of these associated groups.

==> reference.tex <==
\bib{MR4175808}{article}{
   author={Akita, Toshiyuki},
   title={The adjoint group of a Coxeter quandle},
   journal={Kyoto J. Math.},
   volume={60},
   date={2020},
   number={4},
   pages={1245--1260},
   issn={2156-2261},
   review={\MR{4175808}},
   doi={10.1215/21562261-2019-0061},
}


\bib{MR4564617}{article}{
   author={Akita, Toshiyuki},
   title={Embedding Alexander quandles into groups},
   journal={J. Knot Theory Ramifications},
   volume={32},
   date={2023},
   number={2},
   pages={Paper No. 2350011, 4},
   issn={0218-2165},
   review={\MR{4564617}},
   doi={10.1142/S0218216523500116},
}

\bib{MR4447657}{article}{
   author={Akita, Toshiyuki},
   author={Hasegawa, Aoi},
   author={Tanno, Masayoshi},
   title={Structure of the associated groups of quandles},
   journal={Kodai Math. J.},
   volume={45},
   date={2022},
   number={2},
   pages={270--281},
   issn={0386-5991},
   review={\MR{4447657}},
   doi={10.2996/kmj45205},
}

\bib{MR4849109}{article}{
   author={Akita, Toshiyuki},
   author={Takase, Sota},
   title={Groups having Wirtinger presentations and the second group
   homology},
   journal={Kobe J. Math.},
   volume={41},
   date={2024},
   pages={33--39},
   issn={0289-9051},
   review={\MR{4849109}},
}


\bib{MR1994219}{article}{
   author={Andruskiewitsch, Nicol\'as},
   author={Gra\~na, Mat\'ias},
   title={From racks to pointed Hopf algebras},
   journal={Adv. Math.},
   volume={178},
   date={2003},
   number={2},
   pages={177--243},
   issn={0001-8708},
   review={\MR{1994219}},
   doi={10.1016/S0001-8708(02)00071-3},
}



\bib{arXiv:2506.23175}{article}{
   author={Bardakov, Valeriy},
   author={Elhamdadi, Mohamed},
   author={Singh, Mahender},
  title={Yang--Baxter Equation and Related Algebraic Structures},
  date={2025},
  eprint={https://arxiv.org/abs/2506.23175},
%note={preprint},
}



\bib{MR4292536}{book}{
   author={Beggs, Edwin J.},
   author={Majid, Shahn},
   title={Quantum Riemannian geometry},
   series={Grundlehren der mathematischen Wissenschaften [Fundamental
   Principles of Mathematical Sciences]},
   volume={355},
   publisher={Springer, Cham},
   date={2020},
%   date={[2020] \copyright 2020},
   pages={xvi+809},
   isbn={978-3-030-30293-1},
   isbn={978-3-030-30294-8},
   review={\MR{4292536}},
   doi={10.1007/978-3-030-30294-8},
}


\bib{MR1990571}{article}{
   author={Carter, J. Scott},
   author={Jelsovsky, Daniel},
   author={Kamada, Seiichi},
   author={Langford, Laurel},
   author={Saito, Masahico},
   title={Quandle cohomology and state-sum invariants of knotted curves and
   surfaces},
   journal={Trans. Amer. Math. Soc.},
   volume={355},
   date={2003},
   number={10},
   pages={3947--3989},
   issn={0002-9947},
   review={\MR{1990571}},
   doi={10.1090/S0002-9947-03-03046-0},
}



\bib{MR2593699}{article}{
   author={Carter, J. Scott},
   author={Oshiro, Kanako},
   author={Saito, Masahico},
   title={Symmetric extensions of dihedral quandles and triple points of
   non-orientable surfaces},
   journal={Topology Appl.},
   volume={157},
   date={2010},
   number={5},
   pages={857--869},
   issn={0166-8641},
   review={\MR{2593699}},
   doi={10.1016/j.topol.2009.12.002},
}


\bib{MR4899477}{article}{
   author={Cazet, Nicholas},
   title={Quandles with one nontrivial column},
   journal={J. Algebra Appl.},
   volume={24},
   date={2025},
   number={8},
   pages={Paper No. 2550201, 17},
   issn={0219-4988},
   review={\MR{4899477}},
   doi={10.1142/S0219498825502019},
}


\bib{MR2672155}{article}{
   author={Clancy, Maura},
   author={Ellis, Graham},
   title={Homology of some Artin and twisted Artin groups},
   journal={J. K-Theory},
   volume={6},
   date={2010},
   number={1},
   pages={171--196},
   issn={1865-2433},
   review={\MR{2672155}},
   doi={10.1017/is008008012jkt090},
}


\bib{MR3079760}{article}{
   author={Clark, W. Edwin},
   author={Elhamdadi, Mohamed},
   author={Hou, Xiang-dong},
   author={Saito, Masahico},
   author={Yeatman, Timothy},
   title={Connected quandles associated with pointed abelian groups},
   journal={Pacific J. Math.},
   volume={264},
   date={2013},
   number={1},
   pages={31--60},
   issn={0030-8730},
   review={\MR{3079760}},
   doi={10.2140/pjm.2013.264.31},
}


\bib{MR3689901}{article}{
   author={Damiani, Celeste},
   title={A journey through loop braid groups},
   journal={Expo. Math.},
   volume={35},
   date={2017},
   number={3},
   pages={252--285},
   issn={0723-0869},
   review={\MR{3689901}},
   doi={10.1016/j.exmath.2016.12.003},
}



\bib{MR4669143}{article}{
   author={Dhanwani, Neeraj K.},
   author={Raundal, Hitesh R.},
   author={Singh, Mahender},
   title={Dehn quandles of groups and orientable surfaces},
   journal={Fund. Math.},
   volume={263},
   date={2023},
   number={2},
   pages={167--201},
   issn={0016-2736},
   review={\MR{4669143}},
   doi={10.4064/fm271-6-2023},
}



\bib{MR3205568}{article}{
   author={Eisermann, Michael},
   title={Quandle coverings and their Galois correspondence},
   journal={Fund. Math.},
   volume={225},
   date={2014},
   number={1},
   pages={103--168},
   issn={0016-2736},
   review={\MR{3205568}},
   doi={10.4064/fm225-1-7},
}


\bib{MR3671570}{article}{
   author={Garc\'ia Iglesias, Agust\'in},
   author={Vendramin, Leandro},
   title={An explicit description of the second cohomology group of a
   quandle},
   journal={Math. Z.},
   volume={286},
   date={2017},
   number={3-4},
   pages={1041--1063},
   issn={0025-5874},
   review={\MR{3671570}},
   doi={10.1007/s00209-016-1794-7},
}

\bib{MR2365352}{book}{
   author={Geoghegan, Ross},
   title={Topological methods in group theory},
   series={Graduate Texts in Mathematics},
   volume={243},
   publisher={Springer, New York},
   date={2008},
   pages={xiv+473},
   isbn={978-0-387-74611-1},
   review={\MR{2365352}},
   doi={10.1007/978-0-387-74614-2},
}


\bib{MR2803792}{article}{
   author={Gra\~na, M.},
   author={Heckenberger, I.},
   author={Vendramin, L.},
   title={Nichols algebras of group type with many quadratic relations},
   journal={Adv. Math.},
   volume={227},
   date={2011},
   number={5},
   pages={1956--1989},
   issn={0001-8708},
   review={\MR{2803792}},
   doi={10.1016/j.aim.2011.04.006},
}


\bib{hasegawa-thesis}{thesis}{
author={Hasegawa, Aoi},
title={Associated groups of involutive quandles and their second quandle homology},
   type={Thesis (Ph.D)--Hokkaido University},
date={2024},
%eprint={http://hdl.handle.net/2115/92198},
   doi={10.14943/doctoral.k15734},
}


\bib{MR2945646}{article}{
   author={Hatakenaka, Eri},
   author={Nosaka, Takefumi},
   title={Some topological aspects of 4-fold symmetric quandle invariants of
   3-manifolds},
   journal={Internat. J. Math.},
   volume={23},
   date={2012},
   number={7},
   pages={1250064, 31},
   issn={0129-167X},
   review={\MR{2945646}},
   doi={10.1142/S0129167X12500644},
}


\bib{MR3276225}{article}{
   author={Heckenberger, Istv\'an},
   author={Vendramin, Leandro},
   title={Nichols algebras over groups with finite root system of rank two
   II},
   journal={J. Group Theory},
   volume={17},
   date={2014},
   number={6},
   pages={1009--1034},
   issn={1433-5883},
   review={\MR{3276225}},
   doi={10.1515/jgth-2014-0024},
}


\bib{MR2219257}{article}{
   author={Henriques, Andr\'e},
   author={Kamnitzer, Joel},
   title={Crystals and coboundary categories},
   journal={Duke Math. J.},
   volume={132},
   date={2006},
   number={2},
   pages={191--216},
   issn={0012-7094},
   review={\MR{2219257}},
   doi={10.1215/S0012-7094-06-13221-0},
}

\bib{Howie}{article}{
   author={Howie, James},
   title={On the asphericity of ribbon disc complements},
   journal={Trans. Amer. Math. Soc.},
   volume={289},
   date={1985},
   number={1},
   pages={281--302},
   issn={0002-9947},
   review={\MR{0779064}},
   doi={10.2307/1999700},
}

\bib{humphreys}{book}{
   author={Humphreys, James E.},
   title={Reflection groups and Coxeter groups},
   series={Cambridge Studies in Advanced Mathematics},
   volume={29},
   publisher={Cambridge University Press},
   place={Cambridge},
   date={1990},
   pages={xii+204},
   isbn={0-521-37510-X},
   review={\MR{1066460 (92h:20002)}},
}



\bib{MR2890467}{article}{
   author={Jang, Yeonhee},
   author={Oshiro, Kanako},
   title={Symmetric quandle colorings for spatial graphs and
   handlebody-links},
   journal={J. Knot Theory Ramifications},
   volume={21},
   date={2012},
   number={4},
   pages={1250050, 16},
   issn={0218-2165},
   review={\MR{2890467}},
   doi={10.1142/S0218216511010024},
}


\bib{MR0638121}{article}{
   author={Joyce, David},
   title={A classifying invariant of knots, the knot quandle},
   journal={J. Pure Appl. Algebra},
   volume={23},
   date={1982},
   number={1},
   pages={37--65},
   issn={0022-4049},
   review={\MR{0638121}},
   doi={10.1016/0022-4049(82)90077-9},
}


\bib{MR2371714}{article}{
   author={Kamada, Seiichi},
   title={Quandles with good involutions, their homologies and knot
   invariants},
   conference={
      title={Intelligence of low dimensional topology 2006},
   },
   book={
      series={Ser. Knots Everything},
      volume={40},
      publisher={World Sci. Publ., Hackensack, NJ},
   },
   isbn={978-981-270-593-8},
   isbn={981-270-593-7},
   date={2007},
   pages={101--108},
   review={\MR{2371714}},
   doi={10.1142/9789812770967\_0013},
}

\bib{MR3363811}{article}{
   author={Kamada, Seiichi},
   title={Quandles and symmetric quandles for higher dimensional knots},
   conference={
      title={Knots in Poland III. Part III},
   },
   book={
      series={Banach Center Publ.},
      volume={103},
      publisher={Polish Acad. Sci. Inst. Math., Warsaw},
   },
   isbn={978-83-86806-26-3},
   date={2014},
   pages={145--158},
   review={\MR{3363811}},
   doi={10.4064/bc103-0-6},
}


\bib{MR3524589}{article}{
   author={Kamada, Seiichi},
   title={Quandles and knot invariants}, % [translation of MR2978543]},
   journal={Sugaku Expositions},
   volume={29},
   date={2016},
   number={1},
   pages={17--39},
   issn={0898-9583},
   review={\MR{3524589}},
}


\bib{MR4312970}{article}{
   author={Kamada, Seiichi},
   title={Tensor products of quandles and 1-handles attached to
   surface-links},
   journal={Topology Appl.},
   volume={301},
   date={2021},
   pages={Paper No. 107520, 18},
   issn={0166-8641},
   review={\MR{4312970}},
   doi={10.1016/j.topol.2020.107520},
}


\bib{MR3402903}{article}{
   author={Kamada, Seiichi},
   author={Kim, Jieon},
   author={Lee, Sang Youl},
   title={Computations of quandle cocycle invariants of surface-links using
   marked graph diagrams},
   journal={J. Knot Theory Ramifications},
   volume={24},
   date={2015},
   number={10},
   pages={1540010, 35},
   issn={0218-2165},
   review={\MR{3402903}},
   doi={10.1142/S0218216515400106},
}


\bib{MR2657689}{article}{
   author={Kamada, Seiichi},
   author={Oshiro, Kanako},
   title={Homology groups of symmetric quandles and cocycle invariants of
   links and surface-links},
   journal={Trans. Amer. Math. Soc.},
   volume={362},
   date={2010},
   number={10},
   pages={5501--5527},
   issn={0002-9947},
   review={\MR{2657689}},
   doi={10.1090/S0002-9947-2010-05131-1},
}




\bib{MR4881590}{article}{
   author={Karmakar, Biswadeep},
   author={Saraf, Deepanshi},
   author={Singh, Mahender},
   title={Generalized (co)homology of symmetric quandles over homogeneous
   Beck modules},
   journal={J. Pure Appl. Algebra},
   volume={229},
   date={2025},
   number={6},
   pages={Paper No. 107956, 31},
   issn={0022-4049},
   review={\MR{4881590}},
   doi={10.1016/j.jpaa.2025.107956},
}


\bib{arXiv:2407.02971}{article}{
    author={Karmakar, Biswadeep},
   author={Saraf, Deepanshi},
   author={Singh, Mahender},
  title={Automorphisms, cohomology and extensions of symmetric quandles},
  date={2024},
  eprint={https://arxiv.org/abs/2407.02971},
%note={preprint},
}



\bib{MR2435235}{book}{
   author={Kassel, Christian},
   author={Turaev, Vladimir},
   title={Braid groups},
   series={Graduate Texts in Mathematics},
   volume={247},
   note={With the graphical assistance of Olivier Dodane},
   publisher={Springer, New York},
   date={2008},
   pages={xii+340},
   isbn={978-0-387-33841-5},
   review={\MR{2435235}},
   doi={10.1007/978-0-387-68548-9},
}

\bib{MR3993765}{article}{
   author={Kishimoto, Daisuke},
   title={Right-angled Coxeter quandles and polyhedral products},
   journal={Proc. Amer. Math. Soc.},
   volume={147},
   date={2019},
   number={9},
   pages={3715--3727},
   issn={0002-9939},
   review={\MR{3993765}},
   doi={10.1090/proc/14534},
}


\bib{Kulikov}{article}{
   author={Kulikov, V. S.},
%      author={Kulikov, Vik. S.},
   title={Alexander polynomials of plane algebraic curves},
   language={Russian, with Russian summary},
   journal={Izv. Ross. Akad. Nauk Ser. Mat.},
   volume={57},
   date={1993},
   number={1},
   pages={76--101},
   issn={1607-0046},
   translation={
      journal={Russian Acad. Sci. Izv. Math.},
      volume={42},
      date={1994},
      number={1},
      pages={67--89},
      issn={1064-5632},
   },
   review={\MR{1220582}},
   doi={10.1070/IM1994v042n01ABEH001534},
} 

\bib{MR1307063}{article}{
   author={Kulikov, V. S.},
   title={Geometric realization of $C$-groups},
   language={Russian, with Russian summary},
   journal={Izv. Ross. Akad. Nauk Ser. Mat.},
   volume={58},
   date={1994},
   number={4},
   pages={194--203},
   issn={1607-0046},
   translation={
      journal={Russian Acad. Sci. Izv. Math.},
      volume={45},
      date={1995},
      number={1},
      pages={197--206},
      issn={1064-5632},
   },
   review={\MR{1307063}},
   doi={10.1070/IM1995v045n01ABEH001627},
}

\bib{MR1841759}{article}{
   author={Kulikov, V. S.},
%   author={Kulikov, Vik. S.},   
   title={Fundamental groups of the complements to submanifolds of a sphere
   of codimension 2},
   language={Russian, with Russian summary},
   journal={Tr. Mat. Inst. Steklova},
   volume={231},
   date={2000},
   pages={284--293},
   issn={0371-9685},
   translation={
      journal={Proc. Steklov Inst. Math.},
      date={2000},
      number={4(231)},
      pages={271--280},
      issn={0081-5438},
   },
   review={\MR{1841759}},
}

\bib{MR1356352}{article}{
   author={Kuz\cprime min, Yu. V.},
   title={On a method for constructing $C$-groups},
   language={Russian, with Russian summary},
   journal={Izv. Ross. Akad. Nauk Ser. Mat.},
   volume={59},
   date={1995},
   number={4},
   pages={105--124},
   issn={1607-0046},
   translation={
      journal={Izv. Math.},
      volume={59},
      date={1995},
      number={4},
      pages={765--783},
      issn={1064-5632},
   },
   review={\MR{1356352}},
   doi={10.1070/IM1995v059n04ABEH000033},
}


\bib{MR1392843}{article}{
   author={Kuz\cprime min, Yu. V.},
   title={Groups of knotted compact surfaces, and central extensions},
   language={Russian, with Russian summary},
   journal={Mat. Sb.},
   volume={187},
   date={1996},
   number={2},
   pages={81--102},
   issn={0368-8666},
   translation={
      journal={Sb. Math.},
      volume={187},
      date={1996},
      number={2},
      pages={237--257},
      issn={1064-5616},
   },
   review={\MR{1392843}},
   doi={10.1070/SM1996v187n02ABEH000110},
}


\bib{arXiv:2407.02955}{article}{
   author={Victoria Lebed},
  title={Conjugation groups and structure groups of quandles},
  date={2024},
  eprint={https://arxiv.org/abs/2407.02955},
%note={preprint},
}


\bib{MR3974961}{article}{
   author={Lebed, Victoria},
   author={Vendramin, Leandro},
   title={On structure groups of set-theoretic solutions to the Yang-Baxter
   equation},
   journal={Proc. Edinb. Math. Soc. (2)},
   volume={62},
   date={2019},
   number={3},
   pages={683--717},
   issn={0013-0915},
   review={\MR{3974961}},
   doi={10.1017/s0013091518000548},
}

\bib{MR3065997}{article}{
   author={Majid, S.},
   author={Rietsch, K.},
   title={Lie theory and coverings of finite groups},
   journal={J. Algebra},
   volume={389},
   date={2013},
   pages={137--150},
   issn={0021-8693},
   review={\MR{3065997}},
   doi={10.1016/j.jalgebra.2013.02.042},
}



\bib{MR0672410}{article}{
   author={Matveev, S. V.},
   title={Distributive groupoids in knot theory},
   language={Russian},
   journal={Mat. Sb. (N.S.)},
   volume={119(161)},
   date={1982},
   number={1},
   pages={78--88, 160},
   issn={0368-8666},
   review={\MR{0672410}},
}


\bib{MR2821435}{article}{
   author={Nosaka, Takefumi},
   title={4-fold symmetric quandle invariants of 3-manifolds},
   journal={Algebr. Geom. Topol.},
   volume={11},
   date={2011},
   number={3},
   pages={1601--1648},
   issn={1472-2747},
   review={\MR{2821435}},
   doi={10.2140/agt.2011.11.1601},
}


\bib{MR3821082}{article}{
   author={Nosaka, Takefumi},
   title={Central extensions of groups and adjoint groups of quandles},
   conference={
      title={Geometry and analysis of discrete groups and hyperbolic spaces},
   },
   book={
      series={RIMS K\^oky\^uroku Bessatsu},
      volume={B66},
      publisher={Res. Inst. Math. Sci. (RIMS), Kyoto},
   },
   date={2017},
   pages={167--184},
   review={\MR{3821082}},
}

\bib{nosaka-book}{book}{
   author={Nosaka, Takefumi},
   title={Quandles and topological pairs},
   series={SpringerBriefs in Mathematics},
   subtitle={Symmetry, knots, and cohomology},
   publisher={Springer, Singapore},
   date={2017},
   pages={ix+136},
   isbn={978-981-10-6792-1},
   isbn={978-981-10-6793-8},
   review={\MR{3729413}},
   doi={10.1007/978-981-10-6793-8},
}


\bib{MR2629767}{article}{
   author={Oshiro, Kanako},
   title={Triple point numbers of surface-links and symmetric quandle
   cocycle invariants},
   journal={Algebr. Geom. Topol.},
   volume={10},
   date={2010},
   number={2},
   pages={853--865},
   issn={1472-2747},
   review={\MR{2629767}},
   doi={10.2140/agt.2010.10.853},
}





\bib{MR2796229}{article}{
   author={Oshiro, Kanako},
   title={Homology groups of trivial quandles with good involutions and
   triple linking numbers of surface-links},
   journal={J. Knot Theory Ramifications},
   volume={20},
   date={2011},
   number={4},
   pages={595--608},
   issn={0218-2165},
   review={\MR{2796229}},
   doi={10.1142/S0218216511009340},
}


\bib{arXiv:2010.09983}{article}{
   author={Oshiro, Kanako},
  title={Quandles versus symmetric quandles for oriented links},
  date={2020},
  eprint={https://arxiv.org/abs/2010.09983},
%note={preprint},
}


\bib{MR2497781}{article}{
   author={Paris, Luis},
   title={Braid groups and Artin groups},
   conference={
      title={Handbook of Teichm\"uller theory. Vol. II},
   },
   book={
      series={IRMA Lect. Math. Theor. Phys.},
      volume={13},
      publisher={Eur. Math. Soc., Z\"urich},
   },
   date={2009},
   pages={389--451},
   review={\MR{2497781}},
   doi={10.4171/055-1/12},
}



\bib{MR1388194}{article}{
   author={Ryder, Hayley},
   title={An algebraic condition to determine whether a knot is prime},
   journal={Math. Proc. Cambridge Philos. Soc.},
   volume={120},
   date={1996},
   number={3},
   pages={385--389},
   issn={0305-0041},
   review={\MR{1388194}},
   doi={10.1017/S0305004100074958},
}


\bib{MR4594919}{article}{
   author={Saito, Masahico},
   author={Zappala, Emanuele},
   title={Extensions of augmented racks and surface ribbon cocycle
   invariants},
   journal={Topology Appl.},
   volume={335},
   date={2023},
   pages={Paper No. 108555, 19},
   issn={0166-8641},
   review={\MR{4594919}},
   doi={10.1016/j.topol.2023.108555},
}


\bib{Simon}{article}{
   author={Simon, Jonathan},
   title={Wirtinger approximations and the knot groups of $F^{n}$ in
   $S^{n+2}$},
   journal={Pacific J. Math.},
   volume={90},
   date={1980},
   number={1},
   pages={177--190},
   issn={0030-8730},
   review={\MR{599329}},
}


\bib{arXiv:1506.02389}{article}{
   author={David Stanovsk\'y},
   title={The origins of involutory quandles},
   date={2015},
  eprint={https://arxiv.org/abs/1506.02389},
%status={preprint},
}


\bib{arXiv:2505.08090}{article}{
   author={Luc Ta},
  title={Equivalences of racks, Legendrian racks, and symmetric racks},
  date={2025},
  eprint={https://arxiv.org/abs/2505.08090},
%note={preprint},
}


\bib{MR3127819}{article}{
   author={Tamaru, Hiroshi},
   title={Two-point homogeneous quandles with prime cardinality},
   journal={J. Math. Soc. Japan},
   volume={65},
   date={2013},
   number={4},
   pages={1117--1134},
   issn={0025-5645},
   review={\MR{3127819}},
   doi={10.2969/jmsj/06541117},
}

\bib{MR4441473}{article}{
   author={Taniguchi, Yuta},
   title={A homogeneous presentation of symmetric quandles},
   journal={J. Pure Appl. Algebra},
   volume={227},
   date={2023},
   number={1},
   pages={Paper No. 107167, 7},
   issn={0022-4049},
   review={\MR{4441473}},
   doi={10.1016/j.jpaa.2022.107167},
}


\bib{MR4688855}{article}{
   author={Taniguchi, Yuta},
   title={Good involutions of generalized Alexander quandles},
   journal={J. Knot Theory Ramifications},
   volume={32},
   date={2023},
   number={12},
   pages={Paper No. 2350081, 7},
   issn={0218-2165},
   review={\MR{4688855}},
   doi={10.1142/S0218216523500815},
}


\begin{comment}
\bib{MR3685034}{article}{
   author={Vendramin, Leandro},
   title={Doubly transitive groups and cyclic quandles},
   journal={J. Math. Soc. Japan},
   volume={69},
   date={2017},
   number={3},
   pages={1051--1057},
   issn={0025-5645},
   review={\MR{3685034}},
   doi={10.2969/jmsj/06931051},
}
\end{comment}

\bib{Yajima}{article}{
   author={Yajima, Takeshi},
   title={Wirtinger presentations of knot groups},
   journal={Proc. Japan Acad.},
   volume={46},
   date={1970},
   number={10},
   pages={suppl. to 46 (1970), no. 9, 997--1000},
   issn={0021-4280},
   review={\MR{0281781}},
}


\bib{MR4766150}{article}{
   author={Yasuda, Jumpei},
   title={Computation of the knot symmetric quandle and its application to
   the plat index of surface-links},
   journal={J. Knot Theory Ramifications},
   volume={33},
   date={2024},
   number={3},
   pages={Paper No. 2450005, 25},
   issn={0218-2165},
   review={\MR{4766150}},
   doi={10.1142/S0218216524500056},
}


\bib{arXiv:2412.20081}{article}{
   author={Yasuda, Jumpei},
%   author={Jumpei Yasuda},
  title={Characterizations of knot groups and knot symmetric quandles of surface-links},
  date={2024},
  eprint={https://arxiv.org/abs/2412.20081},
%note={preprint},
}

